Making ML models fairer through explanations: the case of LimeOut

Algorithmic decisions are now being used on a daily basis, and based on Machine Learning (ML) processes that may be complex and biased. This raises several concerns given the critical impact that biased decisions may have on individuals or on society as a whole. Not only unfair outcomes affect human rights, they also undermine public trust in ML and AI. In this paper we address fairness issues of ML models based on decision outcomes, and we show how the simple idea of "feature dropout" followed by an "ensemble approach" can improve model fairness. To illustrate, we will revisit the case of "LimeOut" that was proposed to tackle "process fairness", which measures a model's reliance on sensitive or discriminatory features. Given a classifier, a dataset and a set of sensitive features, LimeOut first assesses whether the classifier is fair by checking its reliance on sensitive features using "Lime explanations". If deemed unfair, LimeOut then applies feature dropout to obtain a pool of classifiers. These are then combined into an ensemble classifier that was empirically shown to be less dependent on sensitive features without compromising the classifier's accuracy. We present different experiments on multiple datasets and several state of the art classifiers, which show that LimeOut's classifiers improve (or at least maintain) not only process fairness but also other fairness metrics such as individual and group fairness, equal opportunity, and demographic parity.

==> contributions.tex <==

%% Adult
\begin{table*}[!htb]
    \caption{Global explanation of AdaBoost on Adult dataset.}
    \label{tb:exp-adult}
    \footnotesize
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Original (LIME)}   \\
            \hline
            & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            10 & CapitalGain & -18.449067 \\ 
            11 & CapitalLoss & -4.922207 \\ 
            12 & Hoursperweek & 3.297749 \\ 
            1 & Workclass & -0.997601 \\ 
            2 & fnlwgt & -0.890244 \\ 
            5 & \textbf{MaritalStatus} & 0.873829 \\ 
            9 & \textbf{Sex} & 0.694676 \\ 
            4 & Education-Num & -0.603877 \\ 
            7 & Relationship & 0.277705 \\ 
            6 & Occupation & 0.173059 \\ 
            \hline
        \end{tabular}
    \end{subtable}%
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Ensemble (LIME)}   \\
            \hline
             & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            10 & CapitalGain & -19.147673 \\ 
            11 & CapitalLoss & -9.682837 \\ 
            12 & Hoursperweek & 1.173417 \\ 
            2 & fnlwgt & 0.974685 \\ 
            1 & Workclass & -0.423646 \\ 
            4 & Education-Num & -0.259837 \\ 
            9 & \textbf{Sex} & -0.244728 \\ 
            13 & Country & -0.162728 \\ 
            3 & Education & 0.127105 \\ 
            0 & Age & -0.124858 \\             
            \hline
    \end{tabular}
    \end{subtable} 
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Original (SHAP)}   \\
            \hline
            & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            5  & MaritalStatus  & -2.989672 \\ 
            0  & Age  & 1.88969 \\ 
            3  & Education  & 1.685092 \\ 
            7  & Relationship  & 1.355983 \\ 
            12  & Hoursperweek  & 1.289185 \\ 
            10  & CapitalGain  & -0.645524 \\ 
            9  & Sex  & 0.363072 \\ 
            6  & Occupation  & -0.214036 \\ 
            11  & CapitalLoss  & -0.157263 \\ 
            8  & Race  & 0.130017 \\ 
            \hline
        \end{tabular}
    \end{subtable}%
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Ensemble (SHAP)}   \\
            \hline
             & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            0  & Age  & 1.966225 \\ 
            3  & Education  & 1.829358 \\ 
            5  & MaritalStatus  & -1.577084 \\ 
            12  & Hoursperweek  & 1.234953 \\ 
            10  & CapitalGain  & -0.656483 \\ 
            6  & Occupation  & -0.60199 \\ 
            7  & Relationship  & -0.368134 \\ 
            9  & Sex  & 0.270098 \\ 
            11  & CapitalLoss  & -0.15683 \\ 
            8  & Race  & 0.060848 \\ 
            \hline
    \end{tabular}
    \end{subtable}     
\end{table*}

% German
\begin{table*}[!htb]
    \caption{Global explanation of RF on German dataset.}
    \label{tb:exp-german}
    \footnotesize
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Original (LIME)}   \\
            \hline
            & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            19 & \textbf{foreignworker} & 2.664899 \\ 
            13 & otherinstallmentplans & -1.354191 \\ 
            14 & housing & -1.144371 \\ 
            5 & savings & 0.984104 \\ 
            11 & property & -0.648104 \\ 
            3 & purpose & -0.415498 \\ 
            0 & existingchecking & 0.371415 \\ 
            18 & \textbf{telephone} & 0.311451 \\ 
            2 & credithistory & 0.263366 \\ 
            1 & duration & -0.223288 \\ 
            \hline
        \end{tabular}
    \end{subtable}%
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Ensemble (LIME)}   \\
            \hline
             & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            13 & otherinstallmentplans & -1.487604 \\ 
            14 & housing & -1.089726 \\ 
            5 & savings & 0.679195 \\ 
            1 & duration & -0.483643 \\ 
            19 & \textbf{foreignworker} & 0.448643 \\ 
            11 & property & -0.386355 \\ 
            2 & credithistory & 0.258375 \\ 
            16 & job & -0.252046 \\ 
            0 & existingchecking & -0.21358 \\ 
            10 & residencesince & -0.138818 \\            
            \hline
    \end{tabular}
    \end{subtable} 
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Original (SHAP)}   \\
            \hline
            & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            8  & statussex  & -15.648388 \\ 
            2  & credithistory  & 11.517398 \\ 
            12  & age  & -7.219048 \\ 
            0  & existingchecking  & 6.192362 \\ 
            14  & housing  & -4.081103 \\ 
            5  & savings  & -4.079749 \\ 
            7  & installmentrate  & 3.860959 \\ 
            18  & telephone  & 3.762412 \\ 
            13  & otherinstallmentplans  & -3.520389 \\ 
            16  & job  & -3.37511 \\ 
            \hline
        \end{tabular}
    \end{subtable}%
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Ensemble (SHAP)}   \\
            \hline
             & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            0  & existingchecking  & 16.027906 \\ 
            7  & installmentrate  & 6.241019 \\ 
            14  & housing  & -6.06266 \\ 
            11  & property  & 5.793538 \\ 
            12  & age  & -5.735492 \\ 
            2  & credithistory  & 5.374512 \\ 
            15  & existingcredits  & 4.832019 \\ 
            8  & statussex  & -4.338054 \\ 
            10  & residencesince  & 3.935294 \\ 
            3  & purpose  & 3.773062 \\ 
            \hline
    \end{tabular}
    \end{subtable}     
\end{table*}

% HDMA
\begin{table*}[!htb]
    \caption{Global explanation of Bagging on HMDA dataset.}
    \label{tb:exp-hmda}
    \footnotesize
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Original (LIME)}   \\
            \hline
            & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            0 & derived\_loan\_product\_type & 4.798847 \\ 
            19 & balloon\_payment\_desc & 4.624029 \\ 
            13 & intro\_rate\_period & 4.183828 \\ 
            7 & loan\_to\_value\_ratio & 2.824717 \\ 
            18 & balloon\_payment & 2.005847 \\ 
            12 & prepayment\_penalty\_term & 0.683618 \\ 
            4 & reverse\_mortgage & -0.659169 \\ 
            27 & applicant\_age\_above\_62 & 0.532331 \\ 
            1 & \textbf{derived\_ethnicity} & -0.409255 \\ 
            28 & co\_applicant\_age\_above\_62 & -0.333838 \\ 
            20 & property\_value & -0.326801 \\ 
            2 & \textbf{derived\_race} & -0.318802 \\ 
            26 & applicant\_age & -0.304565 \\ 
            11 & loan\_term & 0.270951 \\ 
            14 & negative\_amortization & -0.229379 \\
            \hline
        \end{tabular}
    \end{subtable}%
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Ensemble (LIME)}   \\
            \hline
             & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            0 & derived\_loan\_product\_type & 6.457707 \\ 
            19 & balloon\_payment\_desc & 5.054243 \\ 
            13 & intro\_rate\_period & 4.638744 \\ 
            18 & balloon\_payment & 1.512304 \\ 
            12 & prepayment\_penalty\_term & -1.267424 \\ 
            16 & interest\_only\_payment & 0.777766 \\ 
            7 & loan\_to\_value\_ratio & 0.704758 \\ 
            15 & negative\_amortization\_desc & 0.61936 \\ 
            5 & reverse\_mortgage\_desc & 0.508204 \\ 
            17 & interest\_only\_payment\_desc & -0.393068 \\ 
            24 & applicant\_credit\_score\_type\_desc & -0.379852 \\ 
            14 & negative\_amortization & -0.353717 \\ 
            27 & applicant\_age\_above\_62 & 0.349847 \\ 
            20 & property\_value & -0.316311 \\ 
            23 & applicant\_credit\_score\_type & -0.192114 \\ 
            \hline
    \end{tabular}
    \end{subtable} 
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Original (SHAP)}   \\
            \hline
            & \textbf{Feature} & \textbf{Contribution} \\
            \hline
             0 & derived\_loan\_product\_type & 140.970607 \\ 
            13 & intro\_rate\_period & 99.472985 \\ 
            2 & \textbf{derived\_race} & -19.674767 \\ 
            24 & applicant\_credit\_score\_type\_desc & 18.279872 \\ 
            23 & applicant\_credit\_score\_type & 15.744163 \\ 
            11 & loan\_term & 7.430295 \\ 
            21 & income & 7.00643 \\ 
            20 & property\_value & 5.621575 \\ 
            27 & applicant\_age\_above\_62 & 4.738737 \\ 
            6 & loan\_amount & 3.766341 \\ 
            26 & applicant\_age & -2.458686 \\ 
            9 & discount\_points & 1.4991 \\ 
            3 & \textbf{derived\_sex} & -1.268657 \\ 
            22 & debt\_to\_income\_ratio & 0.672431 \\ 
            7 & loan\_to\_value\_ratio & 0.375914 \\ 
            \hline
        \end{tabular}
    \end{subtable}%
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Ensemble (SHAP)}   \\
            \hline
             & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            0 & derived\_loan\_product\_type & 164.812554 \\ 
            13 & intro\_rate\_period & 97.646799 \\ 
            24 & applicant\_credit\_score\_type\_desc & 32.129271 \\ 
            23 & applicant\_credit\_score\_type & 13.761834 \\ 
            6 & loan\_amount & 9.864098 \\ 
            2 & \textbf{derived\_race} & -9.814182 \\ 
            21 & income & 9.314534 \\ 
            27 & applicant\_age\_above\_62 & 7.85563 \\ 
            20 & property\_value & 5.911085 \\ 
            22 & debt\_to\_income\_ratio & 4.543734 \\ 
            11 & loan\_term & 4.18301 \\ 
            3 & \textbf{derived\_sex} & 3.562639 \\ 
            7 & loan\_to\_value\_ratio & 3.263888 \\ 
            26 & applicant\_age & 2.034898 \\ 
            10 & lender\_credits & 0.969852 \\ 
            \hline
    \end{tabular}
    \end{subtable}     
\end{table*}

% Dataset
\begin{table*}[!htb]
    \caption{Global explanation of AdaBoost on Default dataset.}
    \label{tb:exp-default}
    \footnotesize
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Original (LIME)}   \\
            \hline
            & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            5 & PAY\_0 & 0.014194 \\ 
            3 & \textbf{MARRIAGE} & -0.013986 \\ 
            6 & PAY\_2 & -0.013513 \\ 
            10 & PAY\_6 & -0.011724 \\ 
            17 & PAY\_AMT1 & 0.011664 \\ 
            22 & PAY\_AMT6 & 0.008088 \\ 
            18 & PAY\_AMT2 & 0.007735 \\ 
            7 & PAY\_3 & 0.00735 \\ 
            2 & EDUCATION & 0.0032 \\ 
            1 & \textbf{SEX} & 0.000732 \\ 
            \hline
        \end{tabular}
    \end{subtable}%
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Ensemble (LIME)}   \\
            \hline
             & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            6 & PAY\_2 & -0.024354 \\ 
            5 & PAY\_0 & 0.008862 \\ 
            9 & PAY\_5 & 0.008729 \\ 
            22 & PAY\_AMT6 & -0.00566 \\ 
            0 & LIMIT\_BAL & -0.003584 \\ 
            12 & BILL\_AMT2 & 0.00329 \\ 
            10 & PAY\_6 & -0.00307 \\ 
            4 & AGE & -0.002058 \\ 
            17 & PAY\_AMT1 & 0.001592 \\ 
            7 & PAY\_3 & -0.001492 \\ 
            \hline
    \end{tabular}
    \end{subtable} 
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Original (SHAP)}   \\
            \hline
            & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            5 & PAY\_0 & -0.971467 \\ 
            18 & PAY\_AMT2 & -0.534922 \\ 
            2 & EDUCATION & 0.40942 \\ 
            19 & PAY\_AMT3 & -0.388805 \\ 
            9 & PAY\_5 & -0.183338 \\ 
            10 & PAY\_6 & -0.138061 \\ 
            3 & \textbf{MARRIAGE} & -0.05459 \\ 
            6 & PAY\_2 & -0.049374 \\ 
            7 & PAY\_3 & -0.028258 \\ 
            1 & \textbf{SEX} & -0.001854 \\ 
            \hline
        \end{tabular}
    \end{subtable}%
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Ensemble (SHAP)}   \\
            \hline
             & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            5 & PAY\_0 & -0.881662 \\ 
            18 & PAY\_AMT2 & -0.287319 \\ 
            19 & PAY\_AMT3 & -0.18995 \\ 
            17 & PAY\_AMT1 & -0.185683 \\ 
            2 & EDUCATION & 0.134975 \\ 
            10 & PAY\_6 & -0.127458 \\ 
            9 & PAY\_5 & -0.107884 \\ 
            7 & PAY\_3 & -0.107713 \\ 
            21 & PAY\_AMT5 & -0.098139 \\ 
            8 & PAY\_4 & -0.065382 \\  
            \hline
    \end{tabular}
    \end{subtable}     
\end{table*}

% LSAC 
\begin{table*}[!htb]
    \caption{Global explanation of Bagging on LSAC dataset.}
    \label{tb:exp-lsac}
    \footnotesize
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Original (LIME)}   \\
            \hline
            & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            3 & isPartTime & -12.588169 \\ 
            5 & \textbf{race} & -3.943962 \\ 
            6 & cluster\_tier & -1.873394 \\ 
            2 & DOB\_yr & -1.235803 \\ 
            1 & zgpa & -0.71457 \\ 
            0 & zfygpa & 0.314865 \\ 
            9 & ugpa & 0.123805 \\ 
            7 & family\_income & -0.08999 \\ 
            8 & lsat & -0.07596 \\ 
            4 & \textbf{sex} & -0.068117 \\ 
            \hline
        \end{tabular}
    \end{subtable}%
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Ensemble (LIME)}   \\
            \hline
             & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            3 & isPartTime & -9.294158 \\ 
            6 & cluster\_tier & -3.464014 \\ 
            1 & zgpa & 2.835836 \\ 
            7 & family\_income & -1.292526 \\ 
            2 & DOB\_yr & -0.923861 \\ 
            5 & \textbf{race} & -0.895484 \\ 
            0 & zfygpa & 0.238397 \\ 
            10 & weighted\_lsat\_ugpa & 0.060846 \\ 
            9 & ugpa & -0.055593 \\ 
            4 & \textbf{sex} & -0.041478 \\
            \hline
    \end{tabular}
    \end{subtable} 
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Original (SHAP)}   \\
            \hline
            & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            1 & zgpa & 25.479357 \\ 
            2 & DOB\_yr & -15.891655 \\ 
            0 & zfygpa & 8.781832 \\ 
            10 & weighted\_lsat\_ugpa & -8.102639 \\ 
            4 & sex & -7.297478 \\ 
            6 & cluster\_tier & -4.952597 \\ 
            9 & ugpa & 4.53557 \\ 
            7 & family\_income & -3.413436 \\ 
            3 & isPartTime & 3.408705 \\ 
            5 & race & 2.001693 \\ 

            \hline
        \end{tabular}
    \end{subtable}%
    \begin{subtable}{\linewidth}
        \setlength{\tabcolsep}{1.9pt}
        \begin{tabular}{r|ll}
            \multicolumn{3}{c}{Ensemble (SHAP)}   \\
            \hline
             & \textbf{Feature} & \textbf{Contribution} \\
            \hline
            1 & zgpa & 26.514648 \\ 
            0 & zfygpa & 13.276902 \\ 
            2 & DOB\_yr & -12.479762 \\ 
            9 & ugpa & 3.378477 \\ 
            6 & cluster\_tier & -2.536884 \\ 
            3 & isPartTime & 2.536474 \\ 
            7 & family\_income & -2.205357 \\ 
            4 & sex & -1.54083 \\ 
            10 & weighted\_lsat\_ugpa & 1.227681 \\ 
            8 & lsat & 0.981232 \\ 

            \hline
    \end{tabular}
    \end{subtable}     
\end{table*}


